Contact Points Discovery for Soft-Body Manipulations with Differentiable Physics

Differentiable physics has recently been shown as a powerful tool for solving soft-body manipulation tasks. However, the differentiable physics solver often gets stuck when the initial contact points of the end effectors are sub-optimal or when performing multi-stage tasks that require contact point switching, which often leads to local minima. To address this challenge, we propose a contact point discovery approach (CPDeform) that guides the stand-alone differentiable physics solver to deform various soft-body plasticines. The key idea of our approach is to integrate optimal transport-based contact points discovery into the differentiable physics solver to overcome the local minima from initial contact points or contact switching. On single-stage tasks, our method can automatically find suitable initial contact points based on transport priorities. On complex multi-stage tasks, we can iteratively switch the contact points of end-effectors based on transport priorities. To evaluate the effectiveness of our method, we introduce PlasticineLab-M that extends the existing differentiable physics benchmark PlasticineLab to seven new challenging multi-stage soft-body manipulation tasks. Extensive experimental results suggest that: 1) on multi-stage tasks that are infeasible for the vanilla differentiable physics solver, our approach discovers contact points that efficiently guide the solver to completion; 2) on tasks where the vanilla solver performs sub-optimally or near-optimally, our contact point discovery method performs better than or on par with the manipulation performance obtained with handcrafted contact points.

==> figures/tex_files/fig_double_manipulator_placement.tex <==
\begin{figure}[H]
\centering

\includegraphics[width=0.8\linewidth]{figures/img_files/double_manipulator_placement.png}

\caption{caption for double-manipulator placement. \sz{need to change figure to show multiple poses, where the rejected ones are with low opacity}}
\label{fig:double_manipulator_placement}
\end{figure}

==> figures/tex_files/fig_temporal_contact_point.tex <==
\begin{figure}[H]
\centering

\includegraphics[width=0.8\linewidth]{figures/img_files/contact_point_in_time.pdf} 

\caption{caption for temporal contact point} 
\label{fig:temporal_contact_point}
\end{figure}

==> text/limitation.tex <==
\section{Limitation}
\label{sec:limitation}

In this work, we are motivated by the observation that the completions of manipulation tasks are usually measured through the external appearances (e.g., vision inputs) in practical applications. Correspondingly, our tasks do not require us to know the internal structures of the object templates. Thus, in this work, we assume that object templates have uniform densities. By uniformly sampling particles inside a given 3D shape of mesh representation, we create its corresponding object template that the differentiable physics solver can use for the manipulation tasks. We think that considerations of target shapes (e.g., a cuboid) with varying internal configurations (e.g., non-uniform density) is an interesting future direction.

\textbf{Volume Assumption}. First, we assume that the volumes of the initial and target shapes are similar. Since our tasks use manipulators that are tailored to compressing instead of expanding the soft materials, the initial shape cannot be significantly smaller than the target shape. Conversely, if the initial shape is significantly larger than the target shape, it will require a lot of effort to compress the initial shape into the target shape. As a solution, we can meet this condition by cutting and assembling the initial plasticines. 

\textbf{Topology Assumption}. we assume that the initial and target shapes do not have tremendous topological differences while requiring shape transformation that involves complex motion planning. When this condition is false, the greedy algorithm that finds the best contact points at the current stage could be  limited. For example, consider a task where the initial shape is a straight rope, and the target shape is a rope with knots. In order to complete the task, the rope needs to be folded and wrapped, which might lead to a temporary increment of shape-matching loss for a few stages. The greedy approach is limited because it might be unwilling to accept the temporary increment of the loss. It would potentially arrive at a solution whose general shape is matched with the target rope by omitting the detailed knots. As a possible solution, if we incorporate RL-based algorithms into our approach, the ability to plan globally could allow the differentiable physics solver to overcome the temporary increment of the loss at an intermediate stage and act for the best completion of the task at the final stage. 

Since these limitation cases are not common in our tasks, we did not take those factors into account in this work. We believe they constitute an interesting future direction to explore.
